Estimating and using information in inverse problems

In inverse problems, one attempts to infer spatially variable functions from indirect measurements of a system. To practitioners of inverse problems, the concept of "information" is familiar when discussing key questions such as which parts of the function can be inferred accurately and which cannot. For example, it is generally understood that we can identify system parameters accurately only close to detectors, or along ray paths between sources and detectors, because we have "the most information" for these places. Although referenced in many publications, the "information" that is invoked in such contexts is not a well understood and clearly defined quantity. Herein, we present a definition of information density that is based on the variance of coefficients as derived from a Bayesian reformulation of the inverse problem. We then discuss three areas in which this information density can be useful in practical algorithms for the solution of inverse problems, and illustrate the usefulness in one of these areas -- how to choose the discretization mesh for the function to be reconstructed -- using numerical experiments.

==> graphics/refinement/gnuplot.1 <==
set nokey
set noxtics
set notics

set size 0.7, 1

set vie 0,0

set term png
set output "points.png"
splot [][][0:] "point_list" us 1:2:($4>0.05 ? -1 : 1) pt 5 ps 0.5, \
               "point_list" us 1:2:($4<0.05 ? -1 : 1) pt 7 ps 0.5



==> graphics/regularization/gnuplot.1 <==
set nokey
set noxtics
set notics

set size 0.7, 1

set vie 0,0

set term png
set output "points.png"
splot [][][0:] "point_list" us 1:2:($4>0.05 ? -1 : 1) pt 5 ps 0.5, \
               "point_list" us 1:2:($4<0.05 ? -1 : 1) pt 7 ps 0.5


